Malware Detection at the Edge with Lightweight LLMs: A Performance Evaluation

The rapid evolution of malware attacks calls for the development of innovative detection methods, especially in resource-constrained edge computing. Traditional detection techniques struggle to keep up with modern malware's sophistication and adaptability, prompting a shift towards advanced methodologies like those leveraging Large Language Models (LLMs) for enhanced malware detection. However, deploying LLMs for malware detection directly at edge devices raises several challenges, including ensuring accuracy in constrained environments and addressing edge devices' energy and computational limits. To tackle these challenges, this paper proposes an architecture leveraging lightweight LLMs' strengths while addressing limitations like reduced accuracy and insufficient computational power. To evaluate the effectiveness of the proposed lightweight LLM-based approach for edge computing, we perform an extensive experimental evaluation using several state-of-the-art lightweight LLMs. We test them with several publicly available datasets specifically designed for edge and IoT scenarios and different edge nodes with varying computational power and characteristics.

==> SummaryEdgeLayer.tex <==




 \newpage
% .
% \newpage


% ####################################################################
% ############## LLM + malware /cyber ################################
% ####################################################################
\section{Summary}


\textbf{1.Introduction} 
    Recall the overall picture from the vision and briefly describe the malware.

\textbf{2.Background}

\begin{itemize}
\item Brief introduction on what an LLM is.
\item Brief history (the key point is the transformer breakthrough with "attention is all you need")
\item Thanks to the transformer, we have different typologies of models (encoder, decoder, and both).
\item We explain these typologies but present only the one treated in the paper for each model.
\item Description (larger than the vision) of the SLM exploited in the paper: TinyBERT, distillBERT, tinyLLama, distillGPT-2, distillT5.
\item Datasets. description of the datasets exploited in the paper: X-IIoTID, CIC IoT 2023, Edge-IIoTset, TON-IoT, Aposemat-23(?).
\end{itemize}




\textbf{3.Applications of SLMs in malware detection (related works)}
    As in the vision paper we list the papers that are much closer to our work (there are still only 2/3 works that cope with us) and possibly new surveys.

\textbf{4.Challenges and Opportunities}
We focus on three main challenges (we mentioned this in the vision) 
 \begin{itemize}
    \item Model performance: evaluate the performance of LLMs in edge malware detection, in terms of accuracy is crucial to consider their application.
    \item Feasibility of deploying LLMs—or their distilled or tiny versions—on edge devices. 
    \item Susceptibility to bias. the risk of overfitting during fine-tuning is critical.
 \end{itemize}




\textbf{5 Proposed Architecture: Edge layer focus.}
 \begin{itemize}
    \item Introduction: we mention the vision architecture, but we only focus on the edge device layer in this paper.
    \item Explain a full flow: We will cover the architecture flow with an example (probably the CCTV IP camera). We will update the architecture picture with numbers for each step of the flow.
    
    \item FLOW: 
    \begin{itemize}
        \item Model selection.
        \item The finetune is performed for the model on a specific dataset.
        \item The finetune model is deployed on the edge device.
        \item The device does its work (natural task) and passes the network data to the model, which is entitled to classify whether the data is malign or not.
        \item The output classification performed by the deployed model on the device is sent to the central model for further analysis and knowledge increase.

    \end{itemize}
    \item Model selection: we must explain which model we focus on and why. We will go with all the models, but we should list why.
    \item How we address the challenges 
        \begin{itemize}
        \item C1. For the model evaluation, we consider accuracy and precision for the test and train set.
        \item C2. We deploy or model on a virtual edge device
        \item C3. During the finetune process, we apply the kfold approach to avoid overfitting and check whether the train and test accuracy diverge over a threshold.
        \end{itemize}
\end{itemize}



\textbf{6 experimental result}
First, we give information about our setup 
\begin{itemize}
    \item considered models.
    \item code repository. huggingfaces reference with the PyTorch framework
    \item dataset
    \item machines. Our lab machine, personal computer, and virtual devices are used.
    
\end{itemize}

Then we explain our finetune process 
\begin{itemize}
    \item The pre-trained model selection
    \item We apply transfer learning with fine-tuning to a pretrained model.    
    %,The pre-trained model is applied to transfer learning with fine-tuning.
    \item Task-Specific Head. 
    \item Supervised Training: The model is fine-tuned on a supervised dataset (EdgeIoT) by training it for 4 epochs using an optimizer and loss function. 
    \begin{itemize}
        \item Loss Function: The loss function is $BCEWithLogitsLoss$, which combines a sigmoid activation with binary cross-entropy loss.
        \item Optimization: The optimizer used is AdamW with a learning rate ($lr=2e-5$).
    \end{itemize}

    \item Evaluation Metrics: 
         Training: Accuracy and Loss. 
        Test: Accuracy, Loss, Precision, recall, and F1 score.
\end{itemize}

We show the virtual device configuration.
the overfitting and feature selection techniques used.
Finally, we show our result sets, divided into three main sets.

        zero shot evaluation
        \begin{enumerate}
            \item we perform the classification with the model that is not yet finetune, but "plain".
        \end{enumerate}
     
      
       
       Model accuracy
        \begin{enumerate}
            \item Same-dataset –  model accuracy over the same dataset used to finetuned the SML model. Model trained on dataset D1 and evaluated on dataset D1.
            \item Cross-dataset -  mode accuracy over a different dataset.we finetuned SML on dataset D1 and evaluated the model accuracy on a different dataset D2.
        \end{enumerate}

        Solution feasibility
            \begin{enumerate}
                \item Exploited dockers to set different virtual (edge/IOT) devices.
            \end{enumerate}
    
Additional tests performed:
\begin{itemize}
    \item Detail on: epochs accuracy loss precision recall validation (test+ train).
    \item feature selection/extraction: Lasso, PCA, RFE, random forest e correlation matrix   
    \item Confusion matrix for a single set of label in a dataset.
\end{itemize}



% List of considered models: 
% \begin{itemize}
%     \item distillBERT
%     \item tinyBERT
%     \item distillGPT2
%     \item tinyllama
%     \item tinyT5
% \end{itemize}

% List of considered datasets: 
% \begin{itemize}
%     \item X-IIoTID. 350 mb
    
%     \item Edge-IIoTset. 1.88 gb
    
%     \item TON-IoT. 3.14gb (solo network)
%     Attacks: DoS, DDoS and ransomware, against web applications, IoT gateways and computer systems across the IoT/IIoT network.
    
%     \item CIC IoT dataset 2023. 12,8 gb

%     \item Aposemat-23 [DA VALUTARE] [Fino a 105 gb]
    
% \end{itemize}












% List of considered onboard test:
% \begin{itemize}
%     \item test set plain -> script con un avg di pacchetti  
%     \item real time usage -> CPU, RAM e tempo di detection 
%     \item è possibile farlo in real time senza devastare le performance?
%     \item 
% \end{itemize}







==> Tables/SingleMalwareAccuracy.tex <==
\begin{table}[]
\begin{tabular}{@{}|l|c|c|c|@{}}
\toprule
\textbf{Class}            & \textbf{Precision} & \textbf{Recall} & \textbf{F1-Score} \\ \midrule
0\_Normal                 & 1.0000             & 1.0000          & 1.0000            \\ \midrule
1\_Backdoor               & 1.0000             & 0.9998          & 0.9999            \\ \midrule
1\_DDoS\_HTTP             & 1.0000             & 1.0000          & 1.0000            \\ \midrule
1\_DDoS\_ICMP             & 1.0000             & 1.0000          & 1.0000            \\ \midrule
1\_DDoS\_TCP              & 1.0000             & 1.0000          & 1.0000            \\ \midrule
1\_DDoS\_UDP              & 1.0000             & 1.0000          & 1.0000            \\ \midrule
1\_Fingerprinting         & 0.9945             & 1.0000          & 0.9973            \\ \midrule
1\_MITM                   & 1.0000             & 1.0000          & 1.0000            \\ \midrule
1\_Password               & 0.9989             & 0.9999          & 0.9994            \\ \midrule
1\_Port\_Scanning         & 0.9998             & 0.9998          & 0.9998            \\ \midrule
1\_Ransomware             & 1.0000             & 1.0000          & 1.0000            \\ \midrule
1\_SQL\_injection         & 0.9999             & 1.0000          & 1.0000            \\ \midrule
1\_Uploading              & 1.0000             & 1.0000          & 1.0000            \\ \midrule
1\_Vulnerability\_scanner & 0.9924             & 0.9983          & 0.9953            \\ \midrule
1\_XSS                    & 0.9971             & 0.9757          & 0.9863            \\ \bottomrule
\end{tabular}
\caption{accuracy on single malware for the dataset edgeiot}
\label{tab:singleACC}
\end{table}

==> Tables/malwareDistribution.tex <==




% \begin{table}[htbp]
% \scalebox{0.7}{
%     \centering
%     \begin{tabular}{l|l|r||l|l|r}
%         \toprule
%         \textbf{Dataset} & \textbf{Attack Type} & \textbf{Occurrences}  & \textbf{Dataset} & \textbf{Attack Type} & \textbf{Occurrences} \\
%         \midrule
%         \multirow{15}{*}{EdgeIoT} 
%             & Normal & 1,615,643 \\
%             & DDoS\_UDP & 121,568 \\
%             & DDoS\_ICMP & 116,436 \\
%             & SQL\_injection & 51,203 \\
%             & Password & 50,153 \\
%             & Vulnerability\_scanner & 50,110 \\
%             & DDoS\_TCP & 50,062 \\
%             & DDoS\_HTTP & 49,911 \\
%             & Uploading & 37,634 \\
%             & Backdoor & 24,862 \\
%             & Port\_Scanning & 22,564 \\
%             & XSS & 15,915 \\
%             & Ransomware & 10,925 \\
%             & MITM & 1,214 \\
%             & Fingerprinting & 1,001 \\
%         \midrule
%         \multirow{10}{*}{ToN-IoT}
%             & Scanning & 7,140,161 \\
%             & DDoS & 6,165,008 \\
%             & DoS & 3,375,328 \\
%             & XSS & 2,108,944 \\
%             & Password & 1,718,568 \\
%             & Normal & 796,380 \\
%             & Backdoor & 508,116 \\
%             & Injection & 452,659 \\
%             & Ransomware & 72,805 \\
%             & MITM & 1,052 \\
%         \midrule
%         \multirow{19}{*}{XIoT}
%             & Normal & 421,417 \\
%             & RDOS & 141,261 \\
%             & Scanning\_vulnerability & 52,852 \\
%             & Generic\_scanning & 50,277 \\
%             & BruteForce & 47,241 \\
%             & MQTT\_cloud\_broker\_subscription & 23,524 \\
%             & Discovering\_resources & 23,148 \\
%             & Exfiltration & 22,134 \\
%             & Insider\_malicious & 17,447 \\
%             & Modbus\_register\_reading & 5,953 \\
%             & False\_data\_injection & 5,094 \\
%             & C\&C & 2,863 \\
%             & Dictionary & 2,572 \\
%             & TCP\_Relay & 2,119 \\
%             & Fuzzing & 1,313 \\
%             & Reverse\_shell & 1,016 \\
%             & Crypto-ransomware & 458 \\
%             & MitM & 117 \\
%             & Fake\_notification & 28 \\
%         \midrule
%         \multirow{34}{*}{CIC-23}
%             & DDoS-ICMP\_Flood & 4,072,433 \\
%             & DDoS-UDP\_Flood & 3,063,433 \\
%             & DDoS-TCP\_Flood & 2,544,126 \\
%             & DDoS-PSHACK\_Flood & 2,314,539 \\
%             & DDoS-SYN\_Flood & 2,295,537 \\
%             & DDoS-RSTFINFlood & 2,289,465 \\
%             & DDoS-SynonymousIP\_Flood & 2,035,476 \\
%             & DoS-UDP\_Flood & 1,878,225 \\
%             & DoS-TCP\_Flood & 1,511,850 \\
%             & DoS-SYN\_Flood & 1,147,330 \\
%             & BenignTraffic & 621,600 \\
%             & Mirai-greeth\_flood & 560,655 \\
%             & Mirai-udpplain & 503,463 \\
%             & Mirai-greip\_flood & 425,570 \\
%             & DDoS-ICMP\_Fragmentation & 255,464 \\
%             & MITM-ArpSpoofing & 174,555 \\
%             & DDoS-UDP\_Fragmentation & 162,730 \\
%             & DDoS-ACK\_Fragmentation & 161,534 \\
%             & DNS\_Spoofing & 101,073 \\
%             & Recon-HostDiscovery & 75,916 \\
%             & Recon-OSScan & 55,556 \\
%             & Recon-PortScan & 46,414 \\
%             & DoS-HTTP\_Flood & 40,705 \\
%             & VulnerabilityScan & 21,045 \\
%             & DDoS-HTTP\_Flood & 16,290 \\
%             & DDoS-SlowLoris & 13,177 \\
%             & DictionaryBruteForce & 7,369 \\
%             & BrowserHijacking & 3,341 \\
%             & CommandInjection & 3,094 \\
%             & SqlInjection & 2,993 \\
%             & XSS & 2,149 \\
%             & Backdoor\_Malware & 1,827 \\
%             & Recon-PingSweep & 1,263 \\
%             & Uploading\_Attack & 720 \\
%         \bottomrule
%     \end{tabular}
%     }
%     \caption{Attack Types Distribution Across Different IoT Security Datasets}
%     \label{tab:combined-attacks}
% \end{table}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[]
\scalebox{0.8}{
\begin{tabular}{@{}llccccll@{}}
\toprule
\multicolumn{4}{c}{EdgeIoT}                   & \multicolumn{4}{|c}{ToN-IoT}                                       \\ \midrule
Attack Type               & Occurrences &  &  & \multicolumn{1}{|c|}{Attack Type}              & Occurrences &  &  \\ \midrule
Normal                    & 1,615,643   &  &  & \multicolumn{1}{|l|}{Scanning}                 & 7,140,161   &  &  \\
DDoS\_UDP                 & 121,568     &  &  & \multicolumn{1}{|l|}{DDoS}                     & 6,165,008   &  &  \\
DDoS\_ICMP                & 116,436     &  &  & \multicolumn{1}{|l|}{DoS}                      & 3,375,328   &  &  \\
SQL\_injection            & 51,203      &  &  & \multicolumn{1}{|l|}{XSS}                      & 2,108,944   &  &  \\
Password                  & 50,153      &  &  & \multicolumn{1}{|l|}{Password}                 & 1,718,568   &  &  \\
Vulnerability\_scanner    & 50,110      &  &  & \multicolumn{1}{|l|}{Normal}                   & 796,380     &  &  \\
DDoS\_TCP                 & 50,062      &  &  & \multicolumn{1}{|l|}{Backdoor}                 & 508,116     &  &  \\
DDoS\_HTTP                & 49,911      &  &  & \multicolumn{1}{|l|}{Injection}                & 452,659     &  &  \\
Uploading                 & 37,634      &  &  & \multicolumn{1}{|l|}{Ransomware}               & 72,805      &  &  \\
Backdoor                  & 24,862      &  &  & \multicolumn{1}{|l|}{MITM}                     & 1,052       &  &  \\
Port\_Scanning            & 22,564      &  &  & \multicolumn{1}{|l|}{}                         &             &  &  \\
XSS                       & 15,915      &  &  & \multicolumn{1}{|l|}{}                         &             &  &  \\
Ransomware                & 10,925      &  &  & \multicolumn{1}{|l|}{}                         &             &  &  \\
MITM                      & 1,214       &  &  & \multicolumn{1}{|l|}{}                         &             &  &  \\
Fingerprinting            & 1,001       &  &  & \multicolumn{1}{|l|}{}                         &             &  &  \\ \midrule
\multicolumn{4}{c}{XIoT}                      & \multicolumn{4}{|c|}{CIC-23}                                       \\ \midrule
Attack Type               & Occurrences &  &  & \multicolumn{1}{|c|}{Attack Type}              & Occurrences &  &  \\ \midrule
Normal                    & 421,417     &  &  & \multicolumn{1}{|l|}{DDoS-ICMP\_Flood}         & 4,072,433   &  &  \\
RDOS                      & 141,261     &  &  & \multicolumn{1}{|l|}{DDoS-UDP\_Flood}          & 3,063,433   &  &  \\
Scanning\_vulnerability   & 52,852      &  &  & \multicolumn{1}{|l|}{DDoS-TCP\_Flood}          & 2,544,126   &  &  \\
Generic\_scanning         & 50,277      &  &  & \multicolumn{1}{|l|}{DDoS-PSHACK\_Flood}       & 2,314,539   &  &  \\
BruteForce                & 47,241      &  &  & \multicolumn{1}{|l|}{DDoS-SYN\_Flood}          & 2,295,537   &  &  \\
MQTT\_cloud\_broker\_subscription & 23,524 &  &  & \multicolumn{1}{|l|}{DDoS-RSTFINFlood}         & 2,289,465 &  &  \\
Discovering\_resources            & 23,148 &  &  & \multicolumn{1}{|l|}{DDoS-SynonymousIP\_Flood} & 2,035,476 &  &  \\
Exfiltration              & 22,134      &  &  & \multicolumn{1}{|l|}{DoS-UDP\_Flood}           & 1,878,225   &  &  \\
Insider\_malicious        & 17,447      &  &  & \multicolumn{1}{|l|}{DoS-TCP\_Flood}           & 1,511,850   &  &  \\
Modbus\_register\_reading & 5,953       &  &  & \multicolumn{1}{|l|}{DoS-SYN\_Flood}           & 1,147,330   &  &  \\
False\_data\_injection    & 5,094       &  &  & \multicolumn{1}{|l|}{BenignTraffic}            & 621,600     &  &  \\
C\&C                      & 2,863       &  &  & \multicolumn{1}{|l|}{Mirai-greeth\_flood}      & 560,655     &  &  \\
Dictionary                & 2,572       &  &  & \multicolumn{1}{|l|}{Mirai-udpplain}           & 503,463     &  &  \\
TCP\_Relay                & 2,119       &  &  & \multicolumn{1}{|l|}{Mirai-greip\_flood}       & 425,570     &  &  \\
Fuzzing                   & 1,313       &  &  & \multicolumn{1}{|l|}{DDoS-ICMP\_Fragmentation} & 255,464     &  &  \\
Reverse\_shell            & 1,016       &  &  & \multicolumn{1}{|l|}{MITM-ArpSpoofing}         & 174,555     &  &  \\
Crypto-ransomware         & 458         &  &  & \multicolumn{1}{|l|}{DDoS-UDP\_Fragmentation}  & 162,730     &  &  \\
MitM                      & 117         &  &  & \multicolumn{1}{|l|}{DDoS-ACK\_Fragmentation}  & 161,534     &  &  \\
Fake\_notification        & 28          &  &  & \multicolumn{1}{|l|}{DNS\_Spoofing}            & 101,073     &  &  \\
                          &             &  &  & \multicolumn{1}{|l|}{Recon-HostDiscovery}      & 75,916      &  &  \\
                          &             &  &  & \multicolumn{1}{|l|}{Recon-OSScan}             & 55,556      &  &  \\
                          &             &  &  & \multicolumn{1}{|l|}{Recon-PortScan}           & 46,414      &  &  \\
                          &             &  &  & \multicolumn{1}{|l|}{DoS-HTTP\_Flood}          & 40,705      &  &  \\
                          &             &  &  & \multicolumn{1}{|l|}{VulnerabilityScan}        & 21,045      &  &  \\
                          &             &  &  & \multicolumn{1}{|l|}{DDoS-HTTP\_Flood}         & 16,290      &  &  \\
                          &             &  &  & \multicolumn{1}{|l|}{DDoS-SlowLoris}           & 13,177      &  &  \\
                          &             &  &  & \multicolumn{1}{|l|}{DictionaryBruteForce}     & 7,369       &  &  \\
                          &             &  &  & \multicolumn{1}{|l|}{BrowserHijacking}         & 3,341       &  &  \\
                          &             &  &  & \multicolumn{1}{|l|}{CommandInjection}         & 3,094       &  &  \\
                          &             &  &  & \multicolumn{1}{|l|}{SqlInjection}             & 2,993       &  &  \\
                          &             &  &  & \multicolumn{1}{|l|}{XSS}                      & 2,149       &  &  \\
                          &             &  &  & \multicolumn{1}{|l|}{Backdoor\_Malware}        & 1,827       &  &  \\
                          &             &  &  & \multicolumn{1}{|l|}{Recon-PingSweep}          & 1,263       &  &  \\
                          &             &  &  & \multicolumn{1}{|l|}{Uploading\_Attack}        & 720         &  &  \\ \bottomrule
\end{tabular}%
}
\caption{}
\label{tab:my-table}
\end{table}





% Single tables

% \begin{figure}[htbp]
%     \centering
%     % Left column - CIC table
%     \begin{minipage}{0.48\textwidth}
%         \centering
%         \begin{tabular}{lr}
%             \toprule
%             \textbf{Attack Type} & \textbf{Occurrences} \\
%             \midrule
%             DDoS-ICMP\_Flood & 4,072,433 \\
%             DDoS-UDP\_Flood & 3,063,433 \\
%             DDoS-TCP\_Flood & 2,544,126 \\
%             DDoS-PSHACK\_Flood & 2,314,539 \\
%             DDoS-SYN\_Flood & 2,295,537 \\
%             DDoS-RSTFINFlood & 2,289,465 \\
%             DDoS-SynonymousIP\_Flood & 2,035,476 \\
%             DoS-UDP\_Flood & 1,878,225 \\
%             DoS-TCP\_Flood & 1,511,850 \\
%             DoS-SYN\_Flood & 1,147,330 \\
%             BenignTraffic & 621,600 \\
%             Mirai-greeth\_flood & 560,655 \\
%             Mirai-udpplain & 503,463 \\
%             Mirai-greip\_flood & 425,570 \\
%             DDoS-ICMP\_Fragmentation & 255,464 \\
%             MITM-ArpSpoofing & 174,555 \\
%             DDoS-UDP\_Fragmentation & 162,730 \\
%             DDoS-ACK\_Fragmentation & 161,534 \\
%             DNS\_Spoofing & 101,073 \\
%             Recon-HostDiscovery & 75,916 \\
%             Recon-OSScan & 55,556 \\
%             Recon-PortScan & 46,414 \\
%             DoS-HTTP\_Flood & 40,705 \\
%             VulnerabilityScan & 21,045 \\
%             DDoS-HTTP\_Flood & 16,290 \\
%             DDoS-SlowLoris & 13,177 \\
%             DictionaryBruteForce & 7,369 \\
%             BrowserHijacking & 3,341 \\
%             CommandInjection & 3,094 \\
%             SqlInjection & 2,993 \\
%             XSS & 2,149 \\
%             Backdoor\_Malware & 1,827 \\
%             Recon-PingSweep & 1,263 \\
%             Uploading\_Attack & 720 \\
%             \bottomrule
%         \end{tabular}
%         \caption{CIC-23 Dataset}
%         \label{tab:cic23-attacks}
%     \end{minipage}%
%     \hfill
%     % Right column - three stacked tables
%     \begin{minipage}{0.48\textwidth}
%         \begin{tabular}{lr}
%             \toprule
%             \textbf{Attack Type} & \textbf{Occurrences} \\
%             \midrule
%             Normal & 1,615,643 \\
%             DDoS\_UDP & 121,568 \\
%             DDoS\_ICMP & 116,436 \\
%             SQL\_injection & 51,203 \\
%             Password & 50,153 \\
%             Vulnerability\_scanner & 50,110 \\
%             DDoS\_TCP & 50,062 \\
%             DDoS\_HTTP & 49,911 \\
%             Uploading & 37,634 \\
%             Backdoor & 24,862 \\
%             Port\_Scanning & 22,564 \\
%             XSS & 15,915 \\
%             Ransomware & 10,925 \\
%             MITM & 1,214 \\
%             Fingerprinting & 1,001 \\
%             \bottomrule
%         \end{tabular}
%         \caption{EdgeIoT Dataset}
%         \label{tab:edgeiot-attacks}
        
%         \vspace{0.5cm}
        
%         \begin{tabular}{lr}
%             \toprule
%             \textbf{Attack Type} & \textbf{Occurrences} \\
%             \midrule
%             Scanning & 7,140,161 \\
%             DDoS & 6,165,008 \\
%             DoS & 3,375,328 \\
%             XSS & 2,108,944 \\
%             Password & 1,718,568 \\
%             Normal & 796,380 \\
%             Backdoor & 508,116 \\
%             Injection & 452,659 \\
%             Ransomware & 72,805 \\
%             MITM & 1,052 \\
%             \bottomrule
%         \end{tabular}
%         \caption{ToN-IoT Dataset}
%         \label{tab:toniot-attacks}
        
%         \vspace{0.5cm}
        
%         \begin{tabular}{lr}
%             \toprule
%             \textbf{Attack Type} & \textbf{Occurrences} \\
%             \midrule
%             Normal & 421,417 \\
%             RDOS & 141,261 \\
%             Scanning\_vulnerability & 52,852 \\
%             Generic\_scanning & 50,277 \\
%             BruteForce & 47,241 \\
%             MQTT\_cloud\_broker\_subscription & 23,524 \\
%             Discovering\_resources & 23,148 \\
%             Exfiltration & 22,134 \\
%             Insider\_malicious & 17,447 \\
%             Modbus\_register\_reading & 5,953 \\
%             False\_data\_injection & 5,094 \\
%             C\&C & 2,863 \\
%             Dictionary & 2,572 \\
%             TCP\_Relay & 2,119 \\
%             Fuzzing & 1,313 \\
%             Reverse\_shell & 1,016 \\
%             Crypto-ransomware & 458 \\
%             MitM & 117 \\
%             Fake\_notification & 28 \\
%             \bottomrule
%         \end{tabular}
%         \caption{XIoT Dataset}
%         \label{tab:xiot-attacks}
%     \end{minipage}
% \end{figure}

==> Tables/testTable.tex <==
% \begin{table}[!htbp]

%     \parbox{.40\textwidth}{
%         \centering
%     \begin{tabular}{@{}|l|l|l|l|l|l|l|l|l|l|l|@{}}
%     \toprule
%       \multicolumn{1}{|c|}{Dataset} &
%       \multicolumn{1}{c|}{Accuracy} &
%       \multicolumn{1}{c|}{Precision} &
%       \multicolumn{1}{c|}{Recall} &
%       \multicolumn{1}{c|}{F1-Score}  \\ \midrule
%         X-IIoTID     &  &  &  &  \\ \midrule
%         Edge-IIoTset & 0.7274 & 0.5346 & 0.7274 & 0.6163 \\ \midrule
%         TON-IoT      &  &  &  &  \\ \midrule
%         CIC IoT 2023 &  &  &  &  \\ \bottomrule
%     \end{tabular}
%         \caption{Results for zero-shot test set}\label{tab:zeroshot}
%     }
%     \hfill
%     \parbox{.45\linewidth}{
%         \centering
%     \begin{tabular}{@{}|l|l|l|l|l|l|l|l|l|l|l|@{}}
%     \toprule
%       \multicolumn{1}{|c|}{Dataset} &
%       \multicolumn{1}{c|}{Accuracy} &
%       \multicolumn{1}{c|}{Precision} &
%       \multicolumn{1}{c|}{Recall} &
%       \multicolumn{1}{c|}{F1-Score}  \\ \midrule
%     X-IIoTID     &  &  &  &  \\ \midrule
%     Edge-IIoTset & 0.7274 & 0.5346 & 0.7274 & 0.6163 \\ \midrule
%     TON-IoT      &  &  &  &  \\ \midrule
%     CIC IoT 2023 &  &  &  &  \\ \bottomrule
%     \end{tabular}
%         \caption{Results for zero-shot test set}\label{tab:zeroshot}
%         }
% \end{table}

% \begin{table}[!htbp]
%     \parbox{.40\textwidth}{
%         \centering
%     \begin{tabular}{@{}|l|l|l|l|l|l|l|l|l|l|l|@{}}
%     \toprule
%       \multicolumn{1}{|c|}{Dataset} &
%       \multicolumn{1}{c|}{Accuracy} &
%       \multicolumn{1}{c|}{Precision} &
%       \multicolumn{1}{c|}{Recall} &
%       \multicolumn{1}{c|}{F1-Score}  \\ \midrule
%         X-IIoTID     &  &  &  &  \\ \midrule
%         Edge-IIoTset & 0.7274 & 0.5346 & 0.7274 & 0.6163 \\ \midrule
%         TON-IoT      &  &  &  &  \\ \midrule
%         CIC IoT 2023 &  &  &  &  \\ \bottomrule
%     \end{tabular}
%         \caption{Results for zero-shot test set}\label{tab:zeroshot}
%     }
%     \hfill
%     \parbox{.45\linewidth}{
%         \centering
%     \begin{tabular}{@{}|l|l|l|l|l|l|l|l|l|l|l|@{}}
%     \toprule
%       \multicolumn{1}{|c|}{Dataset} &
%       \multicolumn{1}{c|}{Accuracy} &
%       \multicolumn{1}{c|}{Precision} &
%       \multicolumn{1}{c|}{Recall} &
%       \multicolumn{1}{c|}{F1-Score}  \\ \midrule
%     X-IIoTID     &  &  &  &  \\ \midrule
%     Edge-IIoTset & 0.7274 & 0.5346 & 0.7274 & 0.6163 \\ \midrule
%     TON-IoT      &  &  &  &  \\ \midrule
%     CIC IoT 2023 &  &  &  &  \\ \bottomrule
%     \end{tabular}
%         \caption{Results for zero-shot test set}\label{tab:zeroshot}
%         }
% \end{table}

% \begin{table}[!htbp]

%     \parbox{.40\textwidth}{
%         \centering
%     \begin{tabular}{@{}|l|l|l|l|l|l|l|l|l|l|l|@{}}
%     \toprule
%       \multicolumn{1}{|c|}{Dataset} &
%       \multicolumn{1}{c|}{Accuracy} &
%       \multicolumn{1}{c|}{Precision} &
%       \multicolumn{1}{c|}{Recall} &
%       \multicolumn{1}{c|}{F1-Score}  \\ \midrule
%         X-IIoTID     &  &  &  &  \\ \midrule
%         Edge-IIoTset & 0.7274 & 0.5346 & 0.7274 & 0.6163 \\ \midrule
%         TON-IoT      &  &  &  &  \\ \midrule
%         CIC IoT 2023 &  &  &  &  \\ \bottomrule
%     \end{tabular}
%         \caption{Results for zero-shot test set}\label{tab:zeroshot}
%     }       

% \end{table}


% \begin{table}[!htbp]
%     \parbox{.40\textwidth}{
%         \centering
%         \begin{tabular}{@{}|l|l|l|l|l|l|l|l|l|l|l|@{}}
%         \toprule
%           \multicolumn{1}{|c|}{Model} &
%           \multicolumn{1}{c|}{Accuracy} &
%           \multicolumn{1}{c|}{Precision} &
%           \multicolumn{1}{c|}{Recall} &
%           \multicolumn{1}{c|}{F1-Score}  \\ \midrule
%         distillGPT2 &  &  &  &  \\ \midrule
%         distillbert &  &  &  &  \\ \midrule
%         tinybert    & 0.7284 & 0.5305 & 0.7284 & 0.6139 \\ \midrule
%         Llama &  &  &  &  \\ \midrule
%         distillT5   &  &  &  &  \\ \bottomrule
%         \end{tabular}
%         \caption{Results for zero-shot test set with  CIC}\label{tab:zeroshot}
%     }
%     \hfill
%     \parbox{.45\linewidth}{
%         \centering
%         \begin{tabular}{@{}|l|l|l|l|l|l|l|l|l|l|l|@{}}
%         \toprule
%           \multicolumn{1}{|c|}{Model} &
%           \multicolumn{1}{c|}{Accuracy} &
%           \multicolumn{1}{c|}{Precision} &
%           \multicolumn{1}{c|}{Recall} &
%           \multicolumn{1}{c|}{F1-Score}  \\ \midrule
%         distillGPT2 &  &  &  &  \\ \midrule
%         distillbert &  &  &  &  \\ \midrule
%         tinybert    & 0.7284 & 0.5305 & 0.7284 & 0.6139 \\ \midrule
%         Llama &  &  &  &  \\ \midrule
%         distillT5   &  &  &  &  \\ \bottomrule
%         \end{tabular}
%         \caption{Results for zero-shot test set with  Ton IoT}\label{tab:zeroshot}
%         }
% \end{table}

% \begin{table}[!htbp]
%     \parbox{.40\linewidth}{
%         \centering
%         \begin{tabular}{@{}|l|l|l|l|l|l|l|l|l|l|l|@{}}
%         \toprule
%           \multicolumn{1}{|c|}{Model} &
%           \multicolumn{1}{c|}{Accuracy} &
%           \multicolumn{1}{c|}{Precision} &
%           \multicolumn{1}{c|}{Recall} &
%           \multicolumn{1}{c|}{F1-Score}  \\ \midrule
%         distillGPT2 &  &  &  &  \\ \midrule
%         distillbert &  &  &  &  \\ \midrule
%         tinybert    & 0.7284 & 0.5305 & 0.7284 & 0.6139 \\ \midrule
%         Llama 3.2 1B &  &  &  &  \\ \midrule
%         distillT5   &  &  &  &  \\ \bottomrule
%         \end{tabular}
%         \caption{Results for zero-shot test set with  Edge}\label{tab:zeroshot}
%     }
%     \hfill
%     \parbox{.45\linewidth}{
%         \centering
%         \begin{tabular}{@{}|l|l|l|l|l|l|l|l|l|l|l|@{}}
%         \toprule
%           \multicolumn{1}{|c|}{Model} &
%           \multicolumn{1}{c|}{Accuracy} &
%           \multicolumn{1}{c|}{Precision} &
%           \multicolumn{1}{c|}{Recall} &
%           \multicolumn{1}{c|}{F1-Score}  \\ \midrule
%         distillGPT2 &  &  &  &  \\ \midrule
%         distillbert &  &  &  &  \\ \midrule
%         tinybert    & 0.7284 & 0.5305 & 0.7284 & 0.6139 \\ \midrule
%         Llama 3.2 1B &  &  &  &  \\ \midrule
%         distillT5   &  &  &  &  \\ \bottomrule
%         \end{tabular}
%         \caption{Results for zero-shot test set with  IXIOT}\label{tab:zeroshot}
%         }
% \end{table}






% \documentclass{article}
% \usepackage{booktabs} % Per una tabella più elegante
% \usepackage{multirow} % Per unire celle verticalmente



% \begin{table*}[!htbp]
%  % \resizebox{\textwidth}{!}{%
% \centering
% \caption{Evaluation results. TPR and FNR refer to binary classification. FPR refers to the multi-class task. For PDBERT, FPR is not applicable due to its training objective.}
% \label{tab:evaluation}
% \begin{tabular}{|l|l|c|c|c|c||l|l|c|c|c|c|}
% \toprule

% \midrule
% \textbf{Model} & \textbf{Dataset} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-Score} & \textbf{Model} & \textbf{Dataset} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-Score} \\
% \midrule
% \multirow{7}{*}{LLAMA 3.1 8B} & CWE-125 & 0.72 & 0.28 & 0.00 & \multirow{7}{*}{PDBERT} & CWE-125 & 0.45 & 0.55 & N/A \\
% & CWE-200 & 0.71 & 0.29 & 0.00 &  & CWE-200 & 0.37 & 0.63 & N/A \\
% & CWE-787 & 0.70 & 0.30 & 0.00 &  & CWE-787 & 0.35 & 0.65 & N/A \\
% & CWE-264 & 0.76 & 0.24 & 0.00 &  & CWE-264 & 0.36 & 0.64 & N/A \\
% & CWE-416 & 0.72 & 0.28 & 0.06 &  & CWE-416 & 0.36 & 0.64 & N/A \\
% & CWE-476 & 0.77 & 0.23 & 0.00 &  & CWE-476 & 0.29 & 0.71 & N/A \\
% & CWE-189 & 0.67 & 0.33 & 0.00 &  & CWE-189 & 0.31 & 0.69 & N/A \\
% \midrule
% \multirow{7}{*}{Mistral v0.3 7B} & CWE-125 & 0.19 & 0.81 & 0.00 & \multirow{7}{*}{GPT-4o mini} & CWE-125 & 0.16 & 0.14 & 0.02 \\
% & CWE-200 & 0.13 & 0.87 & 0.00 &  & CWE-200 & 0.00 & 0.41 & 0.00 \\
% & CWE-787 & 0.25 & 0.75 & 0.00 &  & CWE-787 & 0.02 & 0.37 & 0.01 \\
% & CWE-264 & 0.08 & 0.92 & 0.00 &  & CWE-264 & 0.01 & 0.48 & 0.00 \\
% & CWE-416 & 0.08 & 0.92 & 0.00 &  & CWE-416 & 0.03 & 0.57 & 0.01 \\
% & CWE-476 & 0.78 & 0.22 & 0.00 &  & CWE-476 & 0.41 & 0.23 & 0.15 \\
% & CWE-189 & 0.19 & 0.81 & 0.00 &  & CWE-189 & 0.01 & 0.33 & 0.00 \\

% \bottomrule
% \end{tabular}
% % }
% \end{table*}




































% \begin{table}[ht]
%     \parbox{.40\linewidth}{
%         \centering
%         \begin{tabular}{|l|l|l|}
%             \hline
%             person id & seq id & feature vector$_1$  \\\hline
%             1 & 1 & 1 \\
%             1 & 2 & 1 \\ \hline
%             1 & 1 & 1 \\ \hline
%             1 & 1 & 1 \\ \hline

%         \end{tabular}
%         \caption{HRV Dataset \label{HRVtable}}
%     }
%     \hfill
%     \parbox{.45\linewidth}{
%         \centering
%         \begin{tabular}{|l|l|l|l|}
%             \hline
%             person id & seq id & feature vector$_1$ & feature vector$_2$ \\\hline

%             1 & 1 &1 &1  \\
%             1 & 2 & 1&1 \\ \hline
%             1 & 1 &1 &1\\ \hline
%             1 & 1 & 1 &1 \\ \hline
%         \end{tabular}
%         \caption{BAC Dataset \label{BACtable}}}
% \end{table}












 
% \begin{table}
%   \begin{minipage}{.5\linewidth}
%     \centering
%     \begin{tabular}{ *{3}{c} }
%       \toprule
%       \makecell{person \\ id} & \makecell{seq \\ id} & \makecell{feature \\ vector$_1$} \\
%       \midrule
%       1 & 1 & 1 \\
%       1 & 2 & 1 \\
%       1 & 1 & 1 \\
%       1 & 1 & 1 \\
%       \bottomrule
%     \end{tabular}
%     \caption{HRV Dataset}\label{tab:first}
%   \end{minipage}%
%   \begin{minipage}{.5\linewidth}
%     \centering
%     \begin{tabular}{ *{4}{c} }
%       \toprule
%       \makecell{person \\ id} & \makecell{seq \\ id} & \makecell{feature \\ vector$_1$} & \makecell{feature \\ vector$_2$} \\
%       \midrule
%       1 & 1 & 1 & 4 \\
%       1 & 2 & 1 & 3 \\
%       1 & 1 & 1 & 2 \\
%       1 & 1 & 1 & 1 \\
%       \bottomrule
%     \end{tabular}
%     \caption{BAC Dataset}\label{tab:second}
%   \end{minipage}
% \end{table}

% See Table~\ref{tab:first} and Table~\ref{tab:second}\ldots

% \end{document}






% ######ACM tricks
% \documentclass{acm_proc_article-sp}

% \usepackage{caption}
% \usepackage[labelformat=simple,labelsep=colon]{subcaption}

% \newcommand{\tabc}{\stepcounter{table}}
% % \tabc command will be used to increment counter
% % in subtable.
% % add this command in the end of caption of a 
% % subtable but leaving the subcaption of the first subtable.


% \renewcommand{\thesubtable}{Table~\thetable}
% \begin{document}

% \title{Example}

% \maketitle

% \section{one}
% \begin{table*}[!h]
%   \begin{subtable}{\textwidth}
%   \caption{Power Measurements, 1 and 2 Bids}% no \tabc command here
%   \centering
%   \begin{tabular} {| c | c | c | c | c | c | c |}
%     \hline
%         \textbf{Number of Bids} & \multicolumn{3} {|c|} {\textbf{1}} & \multicolumn{3} {|c|} {\textbf{2}} \\
%     \hline
%         Trial       & 1      & 2      & 3       &   1   & 2       & 3    \\
%     \hline
%         Duration    & 5m 59s & 16m 6s & 5m 57s  & 6m 6s & 15m 37s & 6m 59s  \\
%     \hline
%   \end{tabular}
%   \end{subtable}
%   \\[1mm]
%   \begin{subtable}{\textwidth}
%   \caption{Power Measurements, 3 and 4 \tabc} % \tabc command here and
%   % in the subtables following this one in this table environment
%   \centering
%   \begin{tabular} {| c | c | c | c | c | c | c |}
%     \hline
%         \textbf{Number of Bids} & \multicolumn{3} {|c|} {\textbf{3}} & \multicolumn{3} {|c|} {\textbf{4}} \\
%     \hline
%         Trial       & 1      & 2      & 3       &   1   & 2       & 3    \\
%     \hline
%         Duration    & 7m 25s & 16m 7s & 10m 57s & 5m 49s & 16m 8s & 7m 24s  \\
%     \hline
%   \end{tabular}
%   \end{subtable}
%   % Do not use caption here
% \end{table*}
% \end{document}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \begin{table}[]
% \begin{tabular}{@{}|l|c|c|c|@{}}
% \toprule
% \textbf{Class}            & \textbf{Precision} & \textbf{Recall} & \textbf{F1-Score} \\ \midrule
% 0\_Normal                 & 1.0000             & 1.0000          & 1.0000            \\ \midrule
% 1\_Backdoor               & 1.0000             & 0.9998          & 0.9999            \\ \midrule
% 1\_DDoS\_HTTP             & 1.0000             & 1.0000          & 1.0000            \\ \midrule
% 1\_DDoS\_ICMP             & 1.0000             & 1.0000          & 1.0000            \\ \midrule
% 1\_DDoS\_TCP              & 1.0000             & 1.0000          & 1.0000            \\ \midrule
% 1\_DDoS\_UDP              & 1.0000             & 1.0000          & 1.0000            \\ \midrule
% 1\_Fingerprinting         & 0.9945             & 1.0000          & 0.9973            \\ \midrule
% 1\_MITM                   & 1.0000             & 1.0000          & 1.0000            \\ \midrule
% 1\_Password               & 0.9989             & 0.9999          & 0.9994            \\ \midrule
% 1\_Port\_Scanning         & 0.9998             & 0.9998          & 0.9998            \\ \midrule
% 1\_Ransomware             & 1.0000             & 1.0000          & 1.0000            \\ \midrule
% 1\_SQL\_injection         & 0.9999             & 1.0000          & 1.0000            \\ \midrule
% 1\_Uploading              & 1.0000             & 1.0000          & 1.0000            \\ \midrule
% 1\_Vulnerability\_scanner & 0.9924             & 0.9983          & 0.9953            \\ \midrule
% 1\_XSS                    & 0.9971             & 0.9757          & 0.9863            \\ \bottomrule
% \end{tabular}
% \caption{}
% \label{tab:my-table}
% \end{table}


(da non dimenticarmi: cic ha solo una colonna target)

gpt2-ton
Class label | Precision: 1.0000, Recall: 0.9711, F1: 0.9853
Class type | Precision: 0.9936, Recall: 0.9984, F1: 0.9960
Confusion Matrix:
Actual \ Pred label type
label              236        4          
type              0          559        

gpt2-edge
Class Attack_label | Precision: 1.0000, Recall: 0.9950, F1: 0.9975
Class Attack_type | Precision: 1.0000, Recall: 0.9952, F1: 0.9976
Confusion Matrix:
Actual \ Pred Attack_label Attack_type
Attack_label   593        3
Attack_type    0          204

gpt2-xiot
Class class3 | Precision: 0.9602, Recall: 0.9378, F1: 0.9489
Class class1 | Precision: 0.9119, Recall: 0.9952, F1: 0.9517
Confusion Matrix:
Actual \ Pred class3 class1
class3         364        22
class1         15         399

gpt2-cic
Class label | Precision: 1.0000, Recall: 0.0833, F1: 0.1538

---

bert-ton
Class label | Precision: 1.0000, Recall: 1.0000, F1: 1.0000
Class type | Precision: 1.0000, Recall: 1.0000, F1: 1.0000
Confusion Matrix:
Actual \ Pred label type
label          242        0
type           0          560

bert-edge
Class Attack_label | Precision: 1.0000, Recall: 0.9950, F1: 0.9975
Class Attack_type | Precision: 0.9952, Recall: 1.0000, F1: 0.9976
Confusion Matrix:
Actual \ Pred Attack_label Attack_type
Attack_label   593        3
Attack_type    0          204

bert-xiot
Class class3 | Precision: 0.9948, Recall: 0.9896, F1: 0.9922
Class class1 | Precision: 0.9904, Recall: 0.9904, F1: 0.9904
Confusion Matrix:
Actual \ Pred class3 class1
class3         382        4
class1         2          412

bert-cic
Class label | Precision: 1.0000, Recall: 0.0930, F1: 0.1733

---

tiny-ton
Class label | Precision: 1.0000, Recall: 0.5248, F1: 0.6883
Class type | Precision: 0.7793, Recall: 1.0000, F1: 0.8760
Confusion Matrix:
Actual \ Pred label type
label          127        115
type           0          560

tiny-edge
Class Attack_label | Precision: 0.7450, Recall: 1.0000, F1: 0.8539
Class Attack_type | Precision: 0.0000, Recall: 0.0000, F1: 0.0000
Confusion Matrix:
Actual \ Pred Attack_label Attack_type
Attack_label   596        0
Attack_type    204        0

tiny-xiot
Class class3 | Precision: 0.0000, Recall: 0.0000, F1: 0.0000
Class class1 | Precision: 0.5200, Recall: 1.0000, F1: 0.6842
Confusion Matrix:
Actual \ Pred class3 class1
class3         0          386
class1         0          414

tiny-cic
Class label | Precision: 1.0000, Recall: 0.0957, F1: 0.1810

---

t5-ton
Precision: 0.9369, Recall: 0.9404, F1: 0.9386

t5-edge
recision: 0.9757, Recall: 0.9494, F1: 0.9616

t5-xiot
Precision: 0.9703, Recall: 0.9697, F1: 0.9699

t5-cic
Precision: 0.5243, Recall: 0.5153, F1: 0.4992


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \begin{table}[!h]
%     \begin{tabular}{@{}|l|l|c|c|c|c|c|@{}}
%     \toprule
%     \multicolumn{1}{|c|}{Model}                        & \multicolumn{1}{c|}{Dataset}      & CPU usage  & RAM usage & Class. time & Size & Device \\ \midrule
%     \multicolumn{1}{|c|}{\multirow{4}{*}{distillGPT2}} & \multicolumn{1}{c|}{X-IIoTID}     & $\sim$70\% & 750mb     & $\sim$24sec    & 320mb  & raspi3 \\ \cmidrule(l){2-7} 
%     \multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{Edge-IIoTset} & $\sim$70\% & 750mb     & $\sim$24sec    & 320mb  & raspi3 \\ \cmidrule(l){2-7} 
%     \multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{TON-IoT}      & $\sim$70\% & 750mb     & $\sim$24sec    & 320mb  & raspi3      \\ \cmidrule(l){2-7} 
%     \multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{CIC IoT 2023} & $\sim$70\% & 750mb     & $\sim$24sec    & 320mb  & raspi3 \\ \midrule
%     \multirow{4}{*}{distillbert}                       & \multicolumn{1}{c|}{X-IIoTID}     & $\sim$70\% & 600mb     & $\sim$24sec    & 260mb  & raspi3 \\ \cmidrule(l){2-7} 
%                                                        & \multicolumn{1}{c|}{Edge-IIoTset} & $\sim$70\% & 600mb     & $\sim$24sec    & 260mb  & raspi3 \\ \cmidrule(l){2-7} 
%                                                        & \multicolumn{1}{c|}{TON-IoT}      & $\sim$70\% & 600mb     & $\sim$24sec    & 260mb     & raspi3       \\ \cmidrule(l){2-7} 
%                                                        & CIC IoT 2023                      & $\sim$70\% & 600mb     & $\sim$24sec    & 260mb     & raspi3       \\ \midrule
%     \multirow{4}{*}{tinybert}                          & X-IIoTID                          & $\sim$70\% & 380mb     & $\sim$5sec     & 55mb     & raspi3       \\ \cmidrule(l){2-7} 
%                                                        & Edge-IIoTset                      & $\sim$70\% & 380mb     & $\sim$5sec     & 55mb     & raspi3       \\ \cmidrule(l){2-7} 
%                                                        & TON-IoT                           & $\sim$70\% & 380mb     & $\sim$5sec     & 55mb     & raspi3       \\ \cmidrule(l){2-7} 
%                                                        & CIC IoT 2023                      & $\sim$70\% & 380mb     & $\sim$5sec      & 55mb     & raspi3       \\ \midrule
%     \multirow{4}{*}{tinyllama}                         & X-IIoTID                          & $\sim$70\% & 5.5gb     & $\sim$400sec            & 4.6gb     & raspi3       \\ \cmidrule(l){2-7} 
%                                                        & Edge-IIoTset                      & $\sim$70\% & 5.5gb     & $\sim$400sec            & 4.6gb     & raspi3       \\ \cmidrule(l){2-7} 
%                                                        & TON-IoT                           & $\sim$70\% & 5.5gb     & $\sim$400sec            & 4.6gb     & raspi3       \\ \cmidrule(l){2-7} 
%                                                        & CIC IoT 2023                      & $\sim$70\% & 5.5gb     & $\sim$400sec            & 4.6gb     & raspi3       \\ \midrule
%     \multirow{4}{*}{distillT5}                         & X-IIoTID                          & $\sim$70\% & 400mb     & $\sim$2sec            & 60mb     & raspi3       \\ \cmidrule(l){2-7} 
%                                                        & Edge-IIoTset                      & $\sim$70\% & 400mb     & $\sim$2sec            & 60mb     & raspi3       \\ \cmidrule(l){2-7} 
%                                                        & TON-IoT                           & $\sim$70\% & 400mb     & $\sim$2sec            & 60mb     & raspi3       \\ \cmidrule(l){2-7} 
%                                                        & CIC IoT 2023                      & $\sim$70\% & 400mb     & $\sim$2sec            & 60mb     & raspi3       \\ \bottomrule
%     \end{tabular}
%     \vspace{+0.1em}
%     \caption{Results performance for Raspberry Pi 3}
%     \label{}
%     \end{table}
    



% \begin{table}[!h]
%     \begin{tabular}{@{}|l|l|c|c|c|c|c|@{}}
%     \toprule
%     \multicolumn{1}{|c|}{Model}                        & \multicolumn{1}{c|}{Dataset}      & CPU usage  & Time (cpu) & Time (GPU) & device &  \\ \midrule
%     \multicolumn{1}{|c|}{\multirow{4}{*}{distillGPT2}} & \multicolumn{1}{c|}{X-IIoTID}     & $\sim$10\% & $\sim$750ms     & $\sim$150ms    & jetson  &  \\ \cmidrule(l){2-7} 
%     \multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{Edge-IIoTset} & $\sim$10\% & $\sim$750ms     & $\sim$150ms    & jetson  &  \\ \cmidrule(l){2-7} 
%     \multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{TON-IoT}      & $\sim$10\% & $\sim$750ms     & $\sim$150ms    &  jetson &       \\ \cmidrule(l){2-7} 
%     \multicolumn{1}{|c|}{}                             & \multicolumn{1}{c|}{CIC IoT 2023} & $\sim$10\% & $\sim$750ms     & $\sim$150ms    & jetson  &  \\ \midrule
%     \multirow{4}{*}{distillbert}                       & \multicolumn{1}{c|}{X-IIoTID}     & $\sim$10\% & $\sim$750ms     & $\sim$150ms    & jetson  &  \\ \cmidrule(l){2-7} 
%                                                        & \multicolumn{1}{c|}{Edge-IIoTset} & $\sim$10\% & $\sim$750ms     & $\sim$150ms    & jetson  &  \\ \cmidrule(l){2-7} 
%                                                        & \multicolumn{1}{c|}{TON-IoT}      & $\sim$10\% & $\sim$750ms     & $\sim$150ms    &  jetson    &        \\ \cmidrule(l){2-7} 
%                                                        & CIC IoT 2023                      & $\sim$10\% & $\sim$750ms    & $\sim$150ms    &  jetson    &        \\ \midrule
%     \multirow{4}{*}{tinybert}                          & X-IIoTID                          & $\sim$10\% & $\sim$150ms     & $\sim$30ms     &  jetson    &        \\ \cmidrule(l){2-7} 
%                                                        & Edge-IIoTset                      & $\sim$10\% & $\sim$150ms     & $\sim$30ms     &   jetson   &        \\ \cmidrule(l){2-7} 
%                                                        & TON-IoT                           & $\sim$10\% & $\sim$150ms     & $\sim$30ms     & jetson     &        \\ \cmidrule(l){2-7} 
%                                                        & CIC IoT 2023                      & $\sim$10\% & $\sim$150ms     & $\sim$30ms      & jetson     &        \\ \midrule
%     \multirow{4}{*}{tinyllama}                         & X-IIoTID                          & $\sim$10\% & $\sim$15s     & $\sim$3s            &  jetson    &        \\ \cmidrule(l){2-7} 
%                                                        & Edge-IIoTset                      & $\sim$10\% & $\sim$15s     & $\sim$3s            &  jetson    &        \\ \cmidrule(l){2-7} 
%                                                        & TON-IoT                           & $\sim$10\% & $\sim$15s     & $\sim$3s            &  jetson    &        \\ \cmidrule(l){2-7} 
%                                                        & CIC IoT 2023                      & $\sim$10\% & $\sim$15s     & $\sim$3s            &  jetson    &        \\ \midrule
%     \multirow{4}{*}{distillT5}                         & X-IIoTID                          & $\sim$10\% & $\sim$60ms     & $\sim$12ms            &   jetson   &        \\ \cmidrule(l){2-7} 
%                                                        & Edge-IIoTset                      & $\sim$10\% & $\sim$60ms     & $\sim$12ms            &  jetson    &        \\ \cmidrule(l){2-7} 
%                                                        & TON-IoT                           & $\sim$10\% & $\sim$60ms     & $\sim$12ms            &  jetson    &        \\ \cmidrule(l){2-7} 
%                                                        & CIC IoT 2023                      & $\sim$10\% &  $\sim$60ms    & $\sim$12ms            &   jetson   &        \\ \bottomrule
%     \end{tabular}
%     \vspace{+0.1em}
%     \caption{jetson data (ram stats equal to pi3)}
%     \label{}
%     \end{table}
